Diffusion Curriculum: Synthetic-to-Real Data Curriculum via Image-Guided Diffusion

Low-quality or scarce data has posed significant challenges for training deep neural networks in practice. While classical data augmentation cannot contribute very different new data, diffusion models opens up a new door to build self-evolving AI by generating high-quality and diverse synthetic data through text-guided prompts. However, text-only guidance cannot control synthetic images' proximity to the original images, resulting in out-of-distribution data detrimental to the model performance. To overcome the limitation, we study image guidance to achieve a spectrum of interpolations between synthetic and real images. With stronger image guidance, the generated images are similar to the training data but hard to learn. While with weaker image guidance, the synthetic images will be easier for model but contribute to a larger distribution gap with the original data. The generated full spectrum of data enables us to build a novel "Diffusion Curriculum (DisCL)". DisCL adjusts the image guidance level of image synthesis for each training stage: It identifies and focuses on hard samples for the model and assesses the most effective guidance level of synthetic images to improve hard data learning. We apply DisCL to two challenging tasks: long-tail (LT) classification and learning from low-quality data. It focuses on lower-guidance images of high-quality to learn prototypical features as a warm-up of learning higher-guidance images that might be weak on diversity or quality. Extensive experiments showcase a gain of 2.7% and 2.1% in OOD and ID macro-accuracy when applying DisCL to iWildCam dataset. On ImageNet-LT, DisCL improves the base model's tail-class accuracy from 4.4% to 23.64% and leads to a 4.02% improvement in all-class accuracy.

==> Table_tex/cifar_results.tex <==

\begin{table}[t]
\vspace*{0.4cm}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lc|cccc|cccc@{}}
\toprule
& & \multicolumn{8}{c}{\textbf{CIFAR-100-LT}} \\
& & \multicolumn{4}{c|}{\textbf{Imbalance Ratio=100}} & \multicolumn{4}{c}{\textbf{Imbalance Ratio=50}} \\
\textbf{Method}  & \textbf{Curriculum}   &  \textbf{Many}  & \textbf{Medium} & \textbf{Few} & \textbf{Overall} &  \textbf{Many}  & \textbf{Medium} & \textbf{Few} & \textbf{Overall}  \\
\midrule
\small{CE}        &N/A             & 52.86 & 25.34 & 5.49 & 29.02 & 49.60 & 25.41 & 5.33 & 31.72 \\
% \small{CE + \textcolor{teal}{CUDA}} &N/A & 54.55 & 26.07 & 5.43 & 29.02 & 52.29 & 26.17 & 5.53 & 33.13  \\
\small{CE + CUDA} &N/A & \textbf{54.55} & \textbf{26.07} & 5.43 & 29.85 & 52.29 & 26.17 & 5.53 & 33.13  \\
% \small{CE + CUDA} &N/A & 54.55 & 26.07 & 5.43 & 29.02 & 52.29 & 26.17 & 5.53 & 33.13  \\
\textbf{\small{CE + DisCL}}   &  Diverse to Specific   & 53.14 & 25.52 & \textbf{10.65} & \textbf{30.91} & \textbf{53.4} & \textbf{31.69} & \textbf{21.47} & \textbf{36.22} \\
\midrule
\small{\textcolor{orange}{BS}}          &N/A             & 47.87 & 30.07 & 14.41 & 31.61 & 46.01 & 30.76 & 18.55 & 34.82 \\
% \small{\textcolor{orange}{BS} + \textcolor{teal}{CUDA}} &N/A & 48.01 & 32.79 & 15.55 & 33.02 & 46.08 & 32.51 & 22.11 & 36.21  \\
\small{\textcolor{orange}{BS} + CUDA} &N/A & 48.01 & \textbf{32.79} & 15.55 & 33.02 & 46.08 & 32.51 & 22.11 & 36.21  \\
% \small{\textcolor{orange}{BS} + CUDA} &N/A & 48.01 & 32.79 & 15.55 & 33.02 & 46.08 & 32.51 & 22.11 & 36.21  \\
\textbf{\small{\textcolor{orange}{BS} + DisCL}}  &   Diverse to Specific   & \textbf{49.02} & 29.02 & \textbf{19.07} & \textbf{33.08} & \textbf{49.51} & \textbf{32.60} & \textbf{25.58} & \textbf{36.77}\\
\bottomrule
\end{tabular}%
}
\vspace*{-0.2cm}
\caption{
\small{\textcolor{red}{SB: Combine new results of CIFAR-100 and iNat in one table, occupy too much space rn.}
Accuracy (\%) of long-tail classification on CIFAR-100-LT with base model ResNet-10. The best accuracy for overall and classes of \{many, medium, few\} samples is highlighted in \textbf{bold}. Baselines are defined in \S\ref{itemize:inltbaseline}.}}
\vspace*{0.05cm}
\label{tab:cifarmainresults}
\vspace*{-1\baselineskip}
\end{table}

==> Table_tex/inat_results.tex <==

% \begin{table}[t]
% % \vspace*{-0.4cm}
% \centering
% \resizebox{0.8\columnwidth}{!}{%
% \begin{tabular}{lc|cccc@{}}
% \toprule
% & & \multicolumn{4}{c}{\textbf{iNaturalist2018}} \\
% \textbf{Method}  & \textbf{Curriculum}   &  \textbf{Many}  & \textbf{Medium} & \textbf{Few} & \textbf{Overall}  \\
% \midrule
% \small{CE}            &N/A          & 55.02 & 43.40 & 37.33 & 42.20	\\
% % \small{CE + \textcolor{teal}{CUDA}} &N/A & 55.94 & 44.21 & 39.13 & 43.18 \\
% % \small{CE + CUDA} &N/A & 55.94 & 44.21 & 39.13 & 43.18 \\
% \small{CE + CUDA} &N/A & \textbf{55.94} & 44.21 & 39.13 & 43.18 \\
% \textbf{\small{CE + DisCL}}  &   Diverse to Specific    & 54.71 & \textbf{44.37} & \textbf{48.92} & \textbf{47.25}\\
% \midrule
% \small{\textcolor{orange}{BS}}          &N/A             & 46.12 & 49.31 & 50.27 & 49.46	\\
% % \small{\textcolor{orange}{BS} + \textcolor{teal}{CUDA}} &N/A & 48.77 & 49.94 & 50.87 & 50.23 \\
% % \small{\textcolor{orange}{BS} + CUDA} &N/A & 48.77 & 49.94 & 50.87 & 50.23 \\
% \small{\textcolor{orange}{BS} + CUDA} &N/A & \textbf{48.77} & \textbf{49.94} & 50.87 & 50.23 \\
% \textbf{\small{\textcolor{orange}{BS} + DisCL}}   &   Diverse to Specific   & 45.44 & 48.18 & \textbf{53.63} & \textbf{50.30} \\
% \bottomrule
% \end{tabular}%
% }
% \vspace*{-0.2cm}
% \caption{
% \small{Accuracy (\%) of long-tail classification on iNaturalist2018 with base model ResNet-10. The best accuracy is highlighted in \textbf{bold}. Baselines are defined in \S\ref{itemize:inltbaseline}.}}
% \vspace*{0.05cm}
% \label{tab:inatmainresults}
% \vspace*{-1\baselineskip}
% \end{table}



==> Table_tex/iwildcam_vitl.tex <==

\begin{wraptable}{r}[9pt]{0.5\columnwidth}
\vspace{-1.em}
% \vspace*(-\baselineskip)
\centering
\resizebox{0.45\columnwidth}{!}{%
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
                    & \multicolumn{4}{c}{\textbf{iWildCam}} \\
                    & \multicolumn{2}{c|}{\textbf{Without WE}} & \multicolumn{2}{c}{\textbf{With WE}} \\
\midrule
\textbf{Method}     & \textbf{OOD}    & \textbf{ID} & \textbf{OOD}    & \textbf{ID}  \\
\midrule
CLIP (Zero-Shot)             & 12.1   & 11.8   & 12.1   & 11.8   \\
\small{FLYP\(\dagger\) }       & 40.3    & 55.9      &  41.9   & 57.7    \\
\textbf{\small{FLYP + DisCL}}     & \textbf{43.1}    & \textbf{59.6 }   & \textbf{44.8}    & \textbf{60.2}    \\
\bottomrule
\end{tabular}
}
\vspace*{-0.2cm}
\caption{\textcolor{red}{SB: convert this into bar plot and not another table.}\small{F1 Score with CLIP ViT-L/14}}
% \caption{\small{F1 with ViT-L/14}}
\vspace{-.5em}
% The best numbers are in bold. \(\dagger\) indicates our reproduced results based on their code.
% \sh{to do: combine table 3 with other resutls.}
\label{tab:iwildcammainresult_vitl}
% \vspace*{0.05cm}
% \vspace{-1\baselineskip}
% \vspace{-1.5em}
\end{wraptable}

==> Table_tex/poster_longtail.tex <==
% \begin{table}[t]
% \centering
% \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{}lc|cccc|cccc@{}}
% \toprule
% &      & \multicolumn{4}{c|}{\textbf{ImageNet-LT}} & \multicolumn{4}{c}{\textbf{iNaturalist2018}} \\
% \textbf{Method} & \textbf{Curriculum}     
% &  \textbf{Many}  & \textbf{Medium} & \textbf{Few} & \textbf{Overall}   
% &  \textbf{Many}  & \textbf{Medium} & \textbf{Few} & \textbf{Overall}  \\
% \midrule
% \small{CE}    &N/A                   
% & 57.70   & 26.60   & 4.40  & 35.80       
% & 55.02 & 43.40 & 37.33 & 42.20 \\
% \small{CE + CUDA} &N/A   
% &  \textbf{57.49}  & 28.16   & 6.58  & 36.30  
% & \textbf{55.94} & 44.21 & 39.13 & 43.18 \\
% \small{\textbf{CE + DisCL}}    &  Diverse to Specific   
% &  56.78   &  \textbf{30.73}  & \textbf{23.64}  & \textbf{39.82}   
% & 54.71 & \textbf{44.37} & \textbf{48.92} & \textbf{47.25} \\
% \midrule
% \small{\textcolor{orange}{BS}} & N/A    
% & 51.14 & 37.02   & 19.29  & 39.80 
% & 46.12 & 49.31 & 50.27 & 49.46 \\
% \small{\textcolor{orange}{BS} + CUDA} &N/A  
% &  51.16  &  37.35  &  19.28 & 40.03  
% & \textbf{48.77} & \textbf{49.94} & 50.87 & 50.23 \\
% \small{\textbf{\textcolor{orange}{BS} + DisCL}} &  Diverse to Specific 
% &  \textbf{52.68}  & \textbf{37.68}   & \textbf{21.36}  &  \textbf{41.33}
% & 45.44 & 48.18 & \textbf{53.63} & \textbf{50.30} \\
% \bottomrule
% \end{tabular}%
% }
% \vspace*{-0.2cm}
% \end{table}



\begin{table}[ht]
% \vspace*{-0.5cm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lc|cc@{}}
\toprule
 &        & \multicolumn{2}{c}{\textbf{iWildCam}} \\
 \textbf{Method}  & \textbf{Curriculum}     & \textbf{OOD}    & \textbf{ID}  \\
% \midrule
% \small{CLIP (zero-shot)}                &        & 11.0 (-)   & 8.7 (-)    \\
\midrule
\small{LP-FT}         &N/A                           & 34.7 (0.4)    & 49.7 (0.5)    \\
\small{FLYP}       &N/A                    & 35.5 (1.1)    & 52.2 (0.6)    \\
 % & \small{FLYP + ALIA}       &N/A                    & 36.9 (0.3)    & 52.6 (0.4)    \\
% \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ours}}} & \small{{FLYP + DisCL [Adaptive (CLIPScore > 0.25)]}}    & \textbf{38.2 (0.5)} & \textbf{54.3 (1.4)}    \\
\small{\textbf{FLYP + DisCL}}  & Adaptive  & \textbf{38.2 (0.5)} & \textbf{54.3 (1.4)}    \\
\midrule
\small{LP-FT + WE}  &N/A     &  35.7 (0.4)  &   50.2 (0.5)   \\
\small{FLYP + WE}   &N/A    &  36.4 (1.2)  &   52.0 (1.0)   \\
\small{\textbf{FLYP + DisCL + WE}}   & Adaptive    &  \textbf{38.7 (0.4)}  &   \textbf{54.6 (0.7)}   \\
% \midrule
% \small{FLYP + CurAug (Finetuned on FLYP)}         & 35.9 (0.6)    & 52.8 (1.1)    \\ 
\bottomrule
\end{tabular}
}%
\vspace*{-0.2cm}
% \vspace*{0.05cm}
\vspace*{-1\baselineskip}
\end{table}

==> sections/applications.tex <==
\section{Applications}
\label{sec:application}
\vspace*{-0.1cm}

\subsection{Long-Tail (LT) Classification}
% In long-tail (LT) classification, the scarcity of samples in minority classes makes it difficult for models to extract useful features for these classes, leading to models' poor generalization on balanced test set.
% the number of samples for minority classes is extremely limited, which poses challenges for the model to extract useful features from these limited cases. 
% The limited generalization ability results in a bad performance of the model in classification on the test set. 
% To tackle this issue, we design our DisCL method for long-tail learning, described below.
\vspace*{-0.2cm}
\paragraph{Synthetic Data Generation}
% why design diverse prompt -> to generate diverse data
For synthetic data generation, we follow a standard split of tail classes in the studied dataset. Given the real tail-class samples and the associated text prompts, we generate a full spectrum of synthetic data by techniques in \S\ref{sec:s2r}. To mitigate the imbalance among classes, the key is to increase data diversity and quantity for tail classes. We employ a diverse set of textual prompts to achieve the goal\footnote{Text prompts are provided in Appendix~\ref{sec:app_inltprompt}}.
% We aim to generate more diverse data for minority classes for model to learn more and various features to improve generalization. 
% Using predefined sample difficulty and class-wise accuracy, we identify the samples from tail classes as hard samples and generate a full spectrum of synthetic data with defined text prompts. For long-tail task, as we aim to increase the data diversity, we use diverse text prompts to further improve the diversity of visual features. 

\vspace*{-0.3cm}
\paragraph{Generative Curriculum}
% why non-adaptive curriculum -> to learn from diverse data
% In long tail learning, the primary goal of DisCL is to tackle the inherent issue of class imbalance by initially biasing the models' learning towards the underrepresented tail classes. To accomplish this goal, we design a  predetermined, user-defined curriculum that selects diverse synthetic tail data with low image guidance ($\lambda$ closer to 0) at the beginning of training, and gradually selects the monotonically increasing image guidance ($\lambda$ approaching 1), eventually resembling the original task data. We call this curriculum strategy as "Diverse-to-Specific" due to its smooth transition from synthetic to original images. In addition, since the guidance selection follows a set schedule, we categorize this strategy as "non-adaptive" schedule, as illustrated in Fig.~\ref{fig:teaser}.
The generated spectrum of synthetic data provides varying degrees of data diversity: the images generated with text-only guidance display the highest diversity but may suffer from visual discrepancies to the original images, resulting in a distribution gap that may undermine model performance. To bridge the gap, we progressively shift the synthetic data to a task-specific distribution closer to the original images. This yields a non-adaptive \textbf{``Diverse-to-Specific'' curriculum} that starts with synthetic data with a lower guidance scale ($\lambda \rightarrow$  0) and gradually moves toward data of a higher guidance scale ($\lambda \rightarrow$  1).

\vspace*{-0.1cm}
\subsection{Learning from Low-quality Data}
\label{sec:app_iwild}
% We also explore how the DisCL method can help models learn complex visual features from low-quality images, which is a common issue with real-world data. \textit{For example}, images from traffic, motion or wildlife observation cameras often suffer from noise and obscurity, inturn making it difficult for the models to detect and recognize animals. To address this challenge, we tailor DisCL method to enable extraction of discriminative features  under such challenging circumstances.
% We also investigate DisCL's effect on learning challenging visual features from low-quality data. In real-world scenarios, much data suffers from low quality, such as images from traffic cameras, motion cameras, and wildlife observation cameras. For example, camera trap images for wildlife observation can have degraded quality due to animal movement, weather conditions, and other factors. These conditions make it difficult to detect and recognize animals in the images, posing a challenge for models to extract critical visual features. We use this problem to study the effect of our DisCL.
\vspace*{-0.2cm}
The data collected in real-world scenarios may suffer from low qualities, such as obscurity in images from traffic, motion, or wildlife observation cameras. We investigate wildlife observation as an example application of DisCL to enable effective learning under such challenging scenarios.
\vspace*{-0.3cm}
\paragraph{Synthetic Data Generation}
% how to design prompt -> to generate data with prototypical features -> similar features
For low-quality images from camera traps, we aim to generate simpler images containing more prototypical features of the animals that can warm up the training and generalize to more challenging cases. We first identify hard samples based on the ground-truth class probability by a pretrained classifier: a lower probability indicates more difficulty. 
% Based on this assessment, we identify the challenging samples in images from camera traps. 
We vary the image guidance scale to generate a full spectrum of synthetic data for these hard samples, ranging from prototypical to in-the-wild images. The class information is used in the text prompts\footnote{Text prompts are provided in Appendix~\ref{sec:app_wildprompt}.} to steer the diffusion model to generate images relevant to the animals and their wild environment.

\vspace*{-0.3cm}
\paragraph{Generative Curriculum} \label{sec:iwildcamstrategy}\
Training on text-only synthetic data hinders performance due to their distribution gap to the real data and their differences in hardness. A flexible curriculum strategy that integrates both text-only synthetic and real images during training can mitigate this gap. Unlike long-tail classification, various features in the hard samples of low-quality data are not prototypical or generalizable. Synthetic data with higher image guidance can mitigate the issue to some extent but may remain difficult for models to learn from. In contrast, synthetic data with lower image guidance are more prototypical and easier but they are out-of-distribution (OOD) of the real images. 
% Conversely, data with high image guidance levels, while similar to real images, remain difficult for models to learn from. 

A predefined curriculum of image guidance may introduce OOD features at the early stage, causing a distribution shift, or overemphasizing hard and outlier features, downplaying the prototypical patterns. DoCL \citep{zhou2021curriculum} proposed an adaptive curriculum that selects real data for each training stage that can achieve the greatest progress on the original distribution. The curriculum aims to optimize the training dynamics. 
% the strategy adaptively chooses the most beneficial samples to optimize learning and improve performance. 
Inspired by DoCL, we propose an \textbf{adaptive curriculum} to dynamically select the guidance level that helps the model achieve the best improvement on the real data distribution. 
This approach effectively advances the model from learning simple features to mastering more complex and difficult scenarios.
% We adapt this method to dynamically select the guidance level that helps the model achieve the best improvement on the real data distribution. This approach helps the model effectively transition from learning simple features to mastering more complex and difficult ones.

\vspace*{-0.1cm}


